Explanation-Guided Backdoor Poisoning Attacks Against Malware Classifiers

Training pipelines for machine learning (ML) based malware classification often rely on crowdsourced threat feeds, exposing a natural attack injection point. In this paper, we study the susceptibility of feature-based ML malware classifiers to backdoor poisoning attacks, specifically focusing on challenging "clean label" attacks where attackers do not control the sample labeling process. We propose the use of techniques from explainable machine learning to guide the selection of relevant features and values to create effective backdoor triggers in a model-agnostic fashion. Using multiple reference datasets for malware classification, including Windows PE files, PDFs, and Android applications, we demonstrate effective attacks against a diverse set of machine learning models and evaluate the effect of various constraints imposed on the attacker. To demonstrate the feasibility of our backdoor attacks in practice, we create a watermarking utility for Windows PE files that preserves the binary's functionality, and we leverage similar behavior-preserving alteration methodologies for Android and PDF files. Finally, we experiment with potential defensive strategies and show the difficulties of completely defending against these attacks, especially when the attacks blend in with the legitimate sample distribution.

==> sections/defense_orig.tex <==
In the last few years researchers have started tackling the problem of
defending against backdoor attacks against ML
models~\cite{chen_detecting_2018,tran_spectral_2018,liu_fine-pruning_2018,wang_neural_2019}.
Nearly all the defensive approaches proposed until now, however, are
specifically targeted at (computer vision) Deep Neural Network models, and
assume threat models in which the adversary has actively tampered with the
training labels.  These limitations make them hard to adapt to the class of
model-agnostic attacks we are interested in. Here we will discuss a few
representative examples of the currently published works on the subject.  Tran
et al.~\cite{tran_spectral_2018} identify a properly of backdoor attacks called
\emph{Spectral Signatures}. The defensive methodology based on such signatures,
however, relies on the representation of the class containing two
$\epsilon$-spectrally separable subpopulations, and therefore results
successful only when the signatures are computed in the latent space learned by
the convolutional layers of the network.  Chen et
al.~\cite{chen_detecting_2018}, while considering also text classification as a
target domain, similarly rely on the representation learned by the CNN, by
performing k-means clustering on the activations of the last convolutional
layer. Liu et al.~\cite{liu_fine-pruning_2018} proposed defense is based on
combining network fine tuning and neuron pruning, thus making it not applicable
here. Finally, Wang et al.~\cite{wang_neural_2019} introduce a defensive
procedure called NeuralCleanse based on the intuition that in a backdoored
model, the perturbation necessary to induce a misclassification towards the
targeted class should be smaller than that required to obtain different labels.
It is unclear, however, how this approach could be applied to a non-image
recognition, feature-based, scenario, and on a binary classification model.

Protecting machine learning systems from adversarial attacks is known to be an
intrinsically hard problem~\cite{carlini_evaluating_2019}, and we argue that
both the clean-label nature of our attack, and its targeting of a highly
variable data population (benign binaries), only increase the difficulty of the
task. In the following paragraph we will empirically show that currently
available mitigations are often insufficient, and we will leave a deeper and
more detailed defensive analysis for future work.  Before continuing we
highlight that, according to our threat model, the defender (the party who is
training the anti-virus model) is assumed to have full access to:
\begin{enumerate*}[label=(\roman*)]

    \item the training data, which includes the poisoned points;
        
    \item a small set of trusted clean labeled data (this is a common
        assumption in adversarial machine learning defensive works, and fits
        nicely with the current context since security companies often have
        internal data sources);
        
    \item and to know that the adversary is going to target the most relevant
        features for the model. 

\end{enumerate*}

\subsection{Defensive Approach} 

Our first intuition in designing a mitigation system for these attacks was to
use the \clnfp\ drop as an alarm signaling that a dissemination campaign was
poisoning the training data. As shown in \cref{eval} and
\cref{appendix_results}, some of the attack strategies induce a large shift in
the accuracy on the backdoored goodware, for clean models, especially on NNs.
This basic approach, however, presents multiple shortcomings.
\begin{enumerate*}[label=(\roman*)]

    \item It fails when the attacker employs stealthier strategies, such as
        \combined.

    \item It cannot distinguish between adversarially crafted poison samples
        and unseen-before samples. Therefore, the accuracy drop induced by a
        small poison size, such as $1-2\%$, can be easily confused with a
        natural drop in accuracy due to previously unseen data subpopulations.

    \item Even in the more optimistic scenarios, it can provide only an alert,
        being unable to identify the actual backdoored points.

\end{enumerate*}

Successively, we tried tackling the main obstacle rendering common defensive
methodologies inapplicable: the lack of a learned representation space capable
of accentuating the differences between the training data subpopulations.  To
address this issue and obtain a proxy for the neuron learned latent space, we
used the held-out, safe, data to train a clean model, and extracted the SHAP
values for the safe training set from that model.  This allowed us to select a
fixed number of most important features, and reduce the dimensionality of the
training data to that subspace. We then proceeded to standardize the reduced
vector values between $[-1,1]$. 

Using this pre-processed data, we proceeded to apply the Spectral Signature
methodology described in~\cite{tran_spectral_2018}. Additionally, we explored
the effect of hierarchical density based clustering on the reduced space.  We
applied HDBSCAN~\cite{campello_density-based_2013} and analyzed the resulting
clustering using the Silhouette score. This metric, also used for defensive
cluster analysis by~\cite{chen_detecting_2018}, provides an estimate of the
intra-cluster similarity of an element compared to elements from its nearest
neighbouring cluster.  The intuition here, is that backdoored points should end
up being clustered tightly together, making that cluster easier to distinguish
from the others.  Finally, we trained an Isolation Forest on the same
pre-processed feature space. Isolation Forest, first introduced by Liu et
al.~\cite{liu_isolation_2008}, is an algorithm for unsupervised anomaly
detection, which is based on identifying rare and different points, instead of
building a model of a normal sample.

\Cref{tab:mitigations} shows the effect of these three mitigation strategies
over the different models and attack strategies. Two main takeaways emerge from
these empirical results.  First, the Isolation Forest, trained on the reduced
feature space, is often capable of correctly isolating all the backdoored
points with relatively low false positives. Note that this happens exclusively
when Isolation Forest is trained on the transformed dataset. The same model
applied to the original features only a tiny fraction of the backdoored points
($\approx60-70$), thus reinforcing the observation in~\cite{tran_spectral_2018}
that the subpopulations are not sufficiently separable in the original feature
space. Second, none of the filtering techniques we tried was able to isolate
the points attacked with watermarks produced with the \combined\ strategy. This
confirms our initial intuition that, if the adversary is willing to pay the
price in attack success probability, this strategy can be used to generate
stealthy attacks that are extremely difficult to defend against.


\begin{table*}[ht]
\def\arraystretch{1.1}
\centering
\begin{tabular}{c c c c c c c c}
\toprule
\textbf{Target} & \textbf{Strategy} &  \textbf{\atksuccess} & \textbf{Mitigation} & \textbf{New \atksuccess} & \textbf{Poisons Found} & \textbf{GW Removed} \\
\midrule
\multirow{9}{*}{LightGBM} & \multirow{3}{*}{\makecell{LargeAbsSHAP x \\ MinPopulation}} & \multirow{3}{*}{0.5935} &             HDBSCAN & 0.7422 &  3825 & 102251 \\
 & & &  Spectral Signature & 0.7119 &   962 & 45000\\
 & & &  Isolation Forest & & 6000 & 11184\\
\cline{2-7}
 & \multirow{3}{*}{\makecell{LargeAbsSHAP x \\ CountAbsSHAP}} & \multirow{3}{*}{0.5580} &             HDBSCAN & 0.7055 &  3372 & 93430 \\
 & & &  Spectral Signature & 0.6677 &   961 & 44999\\
 & & &  Isolation Forest & & 6000 & 11480\\
\cline{2-7}
 & \multirow{3}{*}{\makecell{Combined Feature \\ Value Selector}} & \multirow{3}{*}{0.8320} &             HDBSCAN & 0.8427 &  1607 & 115282 \\
 & & &  Spectral Signature & 0.7931 &   328 & 45000\\
 & & &  Isolation Forest & & 204 & 8927\\
\midrule
\multirow{6}{*}{EmberNN} & \multirow{3}{*}{\makecell{LargeAbsSHAP x \\ MinPopulation}}  & \multirow{3}{*}{0.4099} &             HDBSCAN & 0.3508 &  3075 & 137597 \\
 & & &  Spectral Signature & 0.6408 &   906 & 45000\\
 & & &  Isolation Forest & & 6000 & 14512 \\
\cline{2-7}
 & \multirow{3}{*}{\makecell{LargeAbsSHAP x \\ CountAbsSHAP}}  & \multirow{3}{*}{0.8340} &             HDBSCAN & 0.5854 &  2499 & 125460 \\
 & & &  Spectral Signature & 0.8631 &   906 & 45000\\
 & & &  Isolation Forest & & 6000 & 15362 \\
\cline{2-7}
 & \multirow{3}{*}{\makecell{Combined Feature \\ Value Selector}}  & \multirow{3}{*}{0.8457} &             HDBSCAN & 0.8950 &  1610 & 120401 \\
 & & &  Spectral Signature & 0.9689 &   904 & 45000\\
 & & &  Isolation Forest & & 175 & 13289 \\
\bottomrule
\end{tabular}

\caption{Mitigation results both models. All attacks were targeted towards the
\numfeasible\ controllable features identified in \cref{feasible}, with a $1\%$
poison set size corresponding to 6000 backdoored benign samples.}

\label{tab:mitigations}
\end{table*}


% TODO: possibly needs a bit of toning down, to make sure it's clear the
% mitigation proposed is just a first step


==> sections/poisoning_orig.tex <==
Before delving into the details of the methodology used in our experiments, we
will introduce some background on static, feature-based malware detection, and
backdoor poisoning attacks.


\subsection{Malware Detection}

The problem of automated malicious software detection has been of great
interest to the security community for many years. We can roughly distinguish
the numerous proposed solutions into two main classes. Dynamic analysis systems
execute binary files in a virtualized, controlled environment, and record the
behavior of the sample looking for indicators of malicious
behaviors~\cite{mandl_anubis_2009,tam_copperdroid:_2015,amos_applying_2013,kirat_malgene_2015,severi_malrec:_2018}.
On the other hand, static analyzers process the executable file without running
it, and extract the features used for classification directly from the binary
and its meta-data. While there are positive and negative arguments for both
approaches, most endpoint security solutions tend to implement static analyzers
due to the strict time constraints under which they usually operate.  With the
shift towards machine learning based classifiers, this second category has been
split into two additional distinct subsets: hand crafted feature based
detectors~\cite{santos_opcode_2013,mariconti_mamadroid_2017,dehghantanha_machine_2018,saxe_deep_2015,anderson_ember:_2018},
and raw-binary
analyzers~\cite{raff_malware_2017,chua_neural_2017,krcal_deep_2018}.  We focus
our study on the first of these subcategories, since, while this may change in
the coming years, at the time of writing hand-crafted feature based classifiers
seem to outperform the competition, produce easier to interpret predictions,
require less computational resources, and have generally greater diffusion in
commercial solutions.

For our experiments we employ the EMBER~\cite{anderson_ember:_2018} dataset.
The reasons behind this choice were multiple. This dataset proved itself to be
highly relevant in the machine learning for security community, and is
currently regarded as a benchmark for malware analysis models.  Moreover, the
dataset is quite recent, and is being actively supported by the maintainers.
Quite relevant is also the accompanying LightGBM~\cite{ke_lightgbm:_2017} model
which, not only has good baseline performances, but offers a perfect attack
target due to the high utilization of Gradient Boosting methods in the
industry.  Since our interest was in developing a methodology that could be
applied to different model architectures commonly employed in feature-based
malware classifiers, we decided to evaluate our approach against a second model
we designed, a Feed-Forward Neural Network. This model, which we call
\emph{EmberNN}, achieves good classification accuracy results, is quite
generic, and mirrors nicely the architectures often used in literature and
real-world applications. 


\subsection{Backdoor Poisoning Attacks}

Adversarial attacks against machine learning models can be broadly split into
two distinct categories: 

\begin{description}

    \item [evasion] attacks, where the goal of the adversary is to
        modify a testing sample by adding a small perturbation such that the
        model is tricked into assigning a wrong class;

    \item [poisoning] attacks, where the adversary is able to tamper
        with the training data, either injecting arbitrary data points, or
        modifying existing ones, in order to cause a misclassification at
        inference time.

\end{description}

The former class has been, and is still being, extensively explored in the
context of computer vision,\footnote{The literature on this subject in recent
    years has grown so large that it is hard to summarize here. The interested
    reader should consider more comprehensive reading lists, such as the one
provided by
\url{https://nicholas.carlini.com/writing/2018/adversarial-machine-learning-reading-list.html}}
and previous research efforts in this direction have also investigated the
applicability of such techniques to the field of malware
classification~\cite{biggio_evasion_2013,grosse_adversarial_2017,suciu_exploring_2019,kolosnjaji_adversarial_2018,yang_malware_2017}.
In this work, we will focus on the latter category which, until now, has not
been studied so thoroughly.  In particular we are interested in backdoor
attacks, a subclass of poisoning attacks where the adversary's goal is to
inject a pattern in the learned representation of the model, which can be
exploited at inference time to control the classification results.  This
variety of poisoning attacks was first introduced in the context of neural
networks for image recognition by~\cite{gu_badnets:_2017}.

Our work was originally inspired
by~\cite{turner_clean-label_2019,shafahi_poison_2018}, that propose attack
strategies free from the reliance on the adversary's ability to modify training
labels (called \emph{clean-label attacks}).  In the setting we examine, in
fact, crowdsourced data often comes with a set of labels determined by third
party analyzers, that are not under direct control of the attacker. Therefore,
the \emph{clean-label} approach is a de-facto necessity, since label-flipping
implies adversarial control of the labeling process and is extremely difficult
to achieve under most threat models.  We note, however, that the notion of
\emph{clean-label} we use in our work differs slightly form the one originally
proposed by the aforementioned papers. In our scenario the attacker's
modifications of the benign binaries may induce a non predictable label change,
since the labeling process is not directly controllable, and happens after the
poison dissemination phase. While the attacker goal is to minimize the number
of these randomized flips, a small percentage of these benign to malicious
switches can be easily accounted for during the dissemination campaign. We will
expand this issue in further detail in \cref{feasible}. 

%In the remainder of the paper we will refer to the specific combination of
%feature and values injected into the model, and used to induce the
%misclassification, as (backdoor) trigger, watermark, or simply backdoor.


\subsection{Explainable Machine Learning Techniques}

The last decade has seen a flourishing of research contributions to the field
of explainable ML, which accompanied the rise in popularity, and utilisation,
of ML models for practical application.  Among the many systems proposed in the
literature, we decided to use SHapley Additive exPlanations
(SHAP)~\cite{lundberg_unified_2017, lundberg_local_2020}. The SHAP methodology,
based on the cooperative game theory concept of Shapley values, has the
objective of explaining the final value of a prediction by attributing a value
to each feature based on the feature's contribution to the prediction. SHAP
merge together multiple relevant model explanation techniques, including
LIME~\cite{ribeiro_why_2016}, and the Integrated Gradients
method~\cite{sundararajan_axiomatic_2017}. 

Our choice was motivate by a series of reasons.  First, SHAP values provide a
completely model agnostic way to determine feature contributions, which enables
us to make our attack portable to any classifier.  Second, the authors of the
papers, provide a high quality
library\footnote{\url{https://github.com/slundberg/shap}}, and a fast
implementation for Gradient Boosting methods directly integrated inside the
official LightGBM
library\footnote{\url{https://github.com/microsoft/LightGBM}}.  Finally, this
technique has already started being used in the adversarial machine learning
domain, albeit to different ends, by \cite{fidel_when_2019}.





==> sections/revision.tex <==
This work was originally submitted to USENIX Security 2020 and received a Major Revision
response, accompanied by multiple insightful comments for which we thank the
reviewers. In this appendix we will enumerate the changes suggested by the
reviewers and explain how we addressed them in the paper.

\subsection{Revision Expectations}

\bigskip
\begin{blockquote}
    (i) Abstract should be improved in order to better convey the problem
    description. In the Introduction, either support your motivation with
    appropriate references or tone down the statements.
\end{blockquote}

In our revision, we have substantially edited the Abstract and Introduction to more 
precisely focus our motivation and problem description.  We acknowledge that our statements were too general in
nature, and we hope this revised version would more clearly qualify the systems
under scrutiny in our work.

In particular, we note that our use case focuses on malware classifiers using static features, and provide additional 
context for why this is an important area of consideration for the security community, given the importance of such 
classifiers as a first line of defense in commercial endpoint solutions.  We have additionally provided some 
motivation for why the case of backdoor poisoning is relevant even in the face of successful evasion attacks, noting 
that backdoor poisoning can offer a broader and more widespread evasion capability across multiple malware samples and target classifiers -- a particularly important concept given that many vendors use the same threat feeds.
Finally, we made some small changes to reflect the addition of experiments on the Contagio (PDF) dataset and Drebin (Android) datasets.


\bigskip
\begin{blockquote}
    (ii) Extend attack to demonstrate that it can also be applied to more
    involved malware detection systems where features are correlated and bound
    to specific semantics, for example, in common approaches for detecting
    Android and PDF malware.
\end{blockquote}

We revised \Cref{method} to explicitly report how our \combined\ strategy
partially handles correlated features in the dataset. Intuitively, the \combined\ strategy selects feature values in the watermark that are already represented in a region of the benign space, and thus the inherent feature correlations are already captured by the approach, as long as we impose some minor restrictions on the features being considers (notably, that they do not have correlations or dependencies outside of the watermark group). Moreover, constraints imposed by the semantics of the original problem space can be handled by imposing additional costs on the constrained areas of the feature space in our \combined\ strategy  (e.g., increasing the SHAP values).  More generally, we would like to highlight that handling feature correlation in adversarial machine learning, both evasion and poisoning attacks, is a  challenge not handled by most of the literature in this space. Previous work follows a similar approach of limiting the features being attacked to those that are manipulatable without significant side effects or correlations~\cite{srndic_practical_2014, grosse_adversarial_2016, grosse_adversarial_2017}.
Moreover, other advanced, and computationally expensive, techniques can also be used to help increasing the number of features available to our attack strategies, while still ensuring behavior preservation, such as \emph{organ harvesting}, proposed by Pierazzi et al.~\cite{pierazzi_intriguing_2020} for adversarial Android malware, or a behavioral \emph{oracle} as used by Xu et al.~\cite{xu_automatically_2016} for PDF files.

In addition, as suggested
by the reviewers, we describe our adaptation of the proposed attack to both Android and PDF malware detection. We refer the reviewers to the discussion in Section~\ref{sec:otherdata} on how to handle the challenges of creating stable watermarks in both of these datasets.

For PDF malware, we used the Mimicus tool to inject the watermark in a set of 35 features reported to be arbitrarily modifiable in the evasion attack setting~\cite{srndic_practical_2014}. To ensure we create feasible PDF files, we leverage the feature editor utility released with Mimicus~\cite{srndic_practical_2014}. The utility re-generates feature vectors after the watermark is inserted in a PDF file and accounts for potential side effects of the watermark.

In the Drebin dataset, we followed the methodology by Grosse et al.~\cite{grosse_adversarial_2016, grosse_adversarial_2017} introduced for evasion attacks by restricting ourselves to only adding new features that could be changed with a single line in the manifest file. Specifically, we considered the subset of features representing  the list of hardware components and permissions requested by the application.

We believe that our adaptation to these representative datasets in the literature suggested by the reviewers demonstrates the generality of our explanation-guided backdoor poisoning attacks. 

\bigskip
\begin{blockquote}
    (iii) Extend the experimental evaluation and consider an additional dataset
    and/or feature set that is more robust against evasion – see comment (b)
    from Reviewer A
\end{blockquote}

Following the previous point, we show in \Cref{feasible} experimental results
obtained by applying our attack to the suggested Contagio (PDF files) and Drebin (Android applications) datasets. We used the machine learning models proposed in the original papers that introduced these datasets: Random Forest~\cite{srndic_practical_2014}, and a linear SVM~\cite{arp_drebin_2014}. We showed that both these models can be poisoned successfully. For instance, at 1.5\% poisoning rate, the attack induces an average 21.09\% \atksuccess, on Contagio for a 30-feature watermark. Even with the challenges of high dimensionality and sparseness in the Drebin dataset, the attack is still remarkably successful: At 2\% poisoning rate, the attack lowers the accuracy of the model on backdoored samples to 42.9\% on average. We also evaluated in Section~\ref{defense} the most successful mitigation, the Isolation Forest, which identifies no poisoning points for Drebin and only 12.5\% poisoning points for Contagio when applied to the full feature space.

These results demonstrate that our attack strategies are generalizable to a wide range of machine learning classification models, including gradient boosting, random forest, support vector machines, and neural networks, in addition to multiple datasets with different feature types and semantics.


\bigskip
\begin{blockquote}
    (iv) Update related work: see comment (c) from Reviewer A
\end{blockquote}

We added the following references suggested by Reviewer A about influencing automated signature generation for worms:


\begin{enumerate}
\item[-] Newsome et al. RAID 2006. Paragraph: Thwarting Signature Learning by
  Training Maliciously.

\item[-] Perdisci et al. S\&P 2006. Misleading Worm Signature Generators Using
  Deliberate Noise Injection.

\item[-] Venkataraman et al. NDSS 2008. Limits of Learning-based Signature Generation with Adversaries.
\end{enumerate}

We also added the following references about poisoning and defending network
anomaly detection systems, e.g.,:

\begin{enumerate}
	

\item[-] Cretu et al. S\&P 2008 Casting out Demons: Sanitizing Training Data for
  Anomaly Sensors

\item[-] Rubinstein et al. IMC 2009 ANTIDOTE: Understanding and Defending
  against Poisoning of Anomaly Detectors.

\item[-] Kloft et al. AISTATS 2010 Online Anomaly Detection under Adversarial
  Impact

\end{enumerate}

We added these references in the first two paragraphs of the Related Work section. 

\subsection{Other Comments}

\bigskip
\begin{blockquote}
	Reviewer A: Repetitions. There are several repetitions when presenting the
	backdoor approach. It would be easier to follow if everything would
	be presented more precisely. Otherwise, the reader looses track of
	how the concepts are combined. For instance, Section 4.1 repeats the
	SHAP approach again before really discussing the feature selection
	approach.
\end{blockquote}

In order to reduce the number of repetitions, and better organize the exposition, \Cref{background} has been expanded to add a paragraph with details regarding the SHAP methodology, while \Cref{method} has been streamlined focusing only on the way SHAP values are used in the attack process. 



\bigskip
\begin{blockquote}
	Reviewer B: On threat models: I don’t see the value added by trying less realistic and fairly easy ones such as “Unrestricted” and its slight variations in the first half of Table 1. If the adversary modifies features arbitrarily, wouldn’t this contradict the claim/goal of preserving functionality? IMHO, it would make a lot more sense to show the feasibility of backdoor poisoning via realistic threat models only (for a constrained adversary that is determined to put effort because the gain outweighs the adversarial cost).
\end{blockquote}

We have modified \Cref{eval} and \Cref{feasible} to focus more on the \feasibleatk\ adversaries, and the evaluation of behavior preserving attacks on the Drebin and Contagio datasets as mentioned above.\\

We would also like to mention that the goal of this work is twofold: we point out a possible new threat vectors in clean label poisoning attacks on outsourced benign binaries, and we introduce explanation-guided backdoor attacks. Despite our field of interest being malware classification, the attack itself is not bound to any specific domain. It is a general methodology to inject backdoors by leveraging the information provided by modern model explanation instruments, which can be applied to any feature-based classifier, regardless of the domain and the possible feature-space to problem-space mapping issues associated therewith. For this reason we believe that the evaluation in the more general \baseatk\ scenario could still be valuable both as a base exploration step, and for researchers wishing to employ the attack in a context where the threat model is more relaxed.


\bigskip
\begin{blockquote}
	Reviewer B: What if the benign PEs come from only well-vetted legitimate vendors instead of crowdsourced collection of PEs from unknown (hence untrustworthy) sources? Such a scenario is not far from reality and it is implementable. It would be useful if the authors clarify their stance on this issue because they seem to take for granted the fact that both benign and malicious PEs are acquired the crowdsourcing way.
\end{blockquote}


Benign software naturally has an extremely high level of variance and a very long tail of samples, especially in the domain of Windows executable. Gathering a representative sample of custom binaries, multiple versions of popular software, software compiled with different compilers, and obtaining all of it from trusted sources is therefore very difficult. On a daily basis, we see an average of tens of thousands of unique goodware samples from VirusTotal and ReversingLabs feeds. By comparison, some well known trusted sources for binaries, such as VirusTotal Monitor and Chocolatey, have on the order of ten thousand samples in total, which makes it infeasible to cover such a large and variable sample space.

We added a comment on this issue in \Cref{intro}.

%As with most poisoning attacks, the adversary has to be able to inject contaminants inside the training set of the victim model for the attack to be carried out. In our paper, we identify dissemination through crowdsourced threat intelligence platforms as means to this end. Please note that this threat vector is only one component of the full attack process, and the explanation-guided backdoor attack we propose could theoretically be used in other contexts with different circumstances. 
%The scenario proposed by the question, together with our assumption that no re-training of the model is possible, would therefore make any poisoning attack infeasible, since the attacker would not have access to any means to inject the contaminants.
%
%There are, however, multiple reasons why we believe this scenario to be hard to implement. \giocomment{Need to complete this}


\bigskip
\begin{blockquote}
	Reviewer C: Figures 1 provides an overview of the attack on the training pipeline. No the far right of the figure it says “Attacker can now submit malware containing the same backdoor”. Is backdoor in this case referring to the “ specially-engineered watermarked features”? Also, since this paper looks at clean-label attacks, does it mean that the attacker has to use the same ‘backdoor’ on clean samples??
	In general, throughout the paper, the terms ‘backdoor’ and ‘watermark’ are used interchangeably. Is this intentional or if there is a clear distinction between the two, this should be clarified in the paper.
\end{blockquote}

We have reworded the paper and added a note to better clarify that we are using the term \emph{backdoor}, \emph{trigger}, and \emph{watermark} interchangeably during the paper. In most forms of backdoor attacks, the same specific pattern, or feature-value assignment, used to poison the training data, is also used to trigger the desired misclassification during testing. Therefore, yes, in our scenarios, the same feature-value assignment is applied to both the clean label goodware points in the training set and the malicious points during testing. Clean-label backdoor attacks, such as the original attack introduced in the computer vision domain~\cite{turner_clean-label_2019}, similarly inject the backdoor pattern to different classes at training and inference time.

%This is the same way that clean-label backdoor attacks operate in other domains, such as computer vision.


\bigskip
\begin{blockquote}
	Reviewer C: From Section 5 onwards, the paper becomes very difficult to read, partially due to the slew of acronyms, lack of justification for evaluation metrics and necessary required knowledge (about LightGBM and EmberNN) from the reader in order to understand and interpret the results.
	On page 8, first column: a list of indicators is presented to the reader, together with a brief definition. However, there is no explanation on how those values are computed. Even more importantly, one cannot properly interpret the results presented in the rest of the paper without knowing the input values for computing the indicators.  
\end{blockquote}

\Cref{eval} has been reworked in order to simplify the metrics used, and explicitly state over which data they are computed. 


\bigskip
\begin{blockquote}
	Reviewer C: Figure 3 presents a side-by-side comparison of LightGBM and EmberNN. Why is the x-axis labelled differently? The labelling in Figure 5 seems to be more consistent. Since the x-axis has been mislabeled, does it also mean that the information presentation is incorrect? 
\end{blockquote}

We would like to note here that there is no mistake in the labeling of the axes in the plot. Figure 3, now \Cref{fig:new_model_test_set_accuracy}, is split into two sections: the first shows the effectiveness of the attack on a LightGBM victim with a fixed backdoor size and with an increasingly large poisoning pool; the second shows the effect on an EmberNN model with a fixed poisoning percentage and an increasingly large backdoor trigger size (intended as the number of features selected for the backdoor generation). The two subplots have different fixed variables because, as we observe in the text, the effectiveness on the neural networks scales much more interestingly with the number of features composing the trigger rather then with the size of the poisoning pool. We have tried to make the distinction more explicit in the caption of the figure.



\bigskip
\begin{blockquote}
	Reviewer C: Page 2, column 2: what is ML explainability? 
\end{blockquote}

With that phrase we are referring to the area of research in Machine Learning focused on the explanation and interpretation of results produced by a ML algorithm. Given the vastness and complexity of the topic, we refer to the following sources for additional information~\cite{molnar2020interpretable, lundberg_unified_2017, lundberg_consistent_2019, lundberg_local_2020}. In our context, however, we are mostly interested in using the methods developed by researchers in that field to obtain a unified, model agnostic, measure of feature importance, with the additional knowledge of the direction towards which a specific feature-value assignments is expected to pull the classifier outcome.

In the paper, we added a subsection of \Cref{background} to better present the tool, SHAP, we use in our work.


\bigskip
\begin{blockquote}
	Reviewer C: This work focuses on poisoning attacks which attempt to influence the ML training process. In the introduction, the authors mentioned that security companies rely on crowdsourced threat feeds to compile a large, diverse stream of data to train their classifiers. The reason for this is because in order to achieve satisfactory performance by ML detectors, a large quantity of labeled binaries is required. My question is the following: since you are arguing that a diverse, large quantity of data is required, wouldn't it be next to impossible for the attacker to have control over the said data sources, introduce the watermarked features and successfully propagate them in order for your proposed clean-label attacks to be successful? 
\end{blockquote}

Poisoning attacks could happen in any scenario in which the training data is, at least partially, under control of the adversary. In our case, since crowdsourced threat intelligence platforms collect executable samples from their users, they act as centralized aggregators for a myriad of distinct third parties. The victim security company would then acquire the data from a few sources, the threat intelligence platforms, instead of directly collecting them from all the original third parties. Therefore, we believe these threat intelligence platforms could be an effective way for an attacker to disseminate the poisoned data. In most of these platforms (e.g., VirusTotal, AlienVault), any authenticated user can submit binary files, and thus it is relatively easy for attackers to inject files poisoned with the watermark. As we discussed, data labeling is not under adversarial control, and this is the reason we consider clean-label attacks. 

We have reworded \Cref{intro} and \Cref{threat} to try making this concept clearer.



\bigskip
\begin{blockquote}
	Reviewer E: - It is not clear how well the models tested here represent state-of-the-art industrial malware detection. 
\end{blockquote}

Given the type of industry we are referring to in this work, it would be extremely hard to have access to the actual models used in production. The models we analyze, except the one we developed -- EmberNN --, are well known benchmarks and achieve decent performance levels, as measured by F1 scores, on their respective datasets. Being this work focused on presenting an adversarial machine learning attack algorithm, it was not a priority for us to employ models achieving the absolute best, state-of-the-art accuracy ratings. More importantly perhaps, the models we used represent a host of very common architectures (Gradient Boosting Trees, Feed-forward Neural Networks, Random Forests, Support Vector Machines),  over three different datasets, which encourages us to believe the underlying methodology would apply to the actual production models.


\bigskip
\begin{blockquote}
	Reviewer E: - Figure 2 is unreadable.
\end{blockquote}

We have removed the figure and explained the concept in the text.


\bigskip
\begin{blockquote}
	Reviewer E: It is very hard to motivate work on backdoor poisoning attacks when it is still so easy to evade malware models without needing any backdoor. The paper doesn't make a convincing case for why we should be focused on a much stronger threat model, when there is nothing close to a solution for the much weaker threat model. Why would an attacker go to the trouble to poison a model with a backdoor (which requires extraordinary access to the training data) when it is so easy to evade an un-backdoored model? Given the strong threat model, I don't understand why the adversary would be limited to clean-label attack. 
\end{blockquote}

Poisoning attacks, are a real concern for any Machine Learning model when an adversary could have any means of access or control over the training set. Early works in this area focusing on computer security date back to 2006, where the goal of the adversary was influencing the automated signature generation for polymorphic worms. Since then, they have been the object of numerous studies, and nowadays are being considered particularly relevant by industry practitioners~\cite{kumar2020adversarial}. We refer to \Cref{relwork} for additional details.

We therefore believe that both poisoning and evasion attacks should be studied when analyzing the security of an ML algorithm. 

% as it happens in the field of Computer Vision and Natural Language Processing,



==> sections/threat_orig.tex <==
{\renewcommand{\arraystretch}{1.05}%
\begin{table}
\small
\centering
\begin{tabularx}{0.5\textwidth}{X|l|l}
\toprule

\textbf{Attacker capabilities} & \textbf{Category} & \textbf{Attack Name} \\ 
\midrule

Can modify any feature, arbitrarily. & white-box & \baseatk \\ \hline

Has knowledge of the features, but not the model. Computation is constrained on
surrogate models. & grey-box & \transferatk \\ \hline

Can modify only a subset of the feature space, using only a subset of the value
space. & white-box & \feasibleatk \\ 
\bottomrule
\end{tabularx}
\caption{Summary of attacker scenarios.}
\label{tab:attacker}
\end{table}
}



Motivated by the widespread applicability of static malware detectors in
industry, our first goal is to investigate the susceptibility of these malware
detectors to backdoor poisoning attacks. A backdoor, also called watermark or
trigger, is a specific pattern, a combination of features and selected values,
injected into the model at training time, used to induce the misclassification
of backdoored points at testing time. We consider several classes of
adversaries, including an attacker with full knowledge of the system and
ability to modify features arbitrarily, as well as more realistic adversaries
with constrained capabilities. We also study to what extent our attacks are
feasible to mount in practice by modifying the real malware binaries to inject
the backdoors in feature space and influence the prediction of exiting malware
detectors. Our last consideration in designing the attacks is their
detectability or stealthiness. In this context, we explore attack strategies
that preserve the legitimate data distribution and become hard to detect with
simple mitigations.

Our second goal is to evaluate existing defensive counter-measures against our
suite of backdoor attacks with different properties, determine when they might
fail, and design more effective mitigations for stealthy poisoning attacks. We
plan to analyze the inherent tradeoffs between the backdoor attacks'
effectiveness, their impact on clean binaries, their practical feasibility, and
the attacks' detectability with the proposed counter-measures.

% During the process, we aim to explore a suite of attack strategies that
% become more and more  undetectable, and several mitigation methods that might
% reduce the risk of backdoor poisoning attacks. 

In the remainder of this section, we detail our adversarial model, the
adversarial goals and capabilities, and mention challenges of designing
poisoning attacks and mitigations against ML-based malware classifiers. 


\subsection{Threat model} 

Given the security sensitive context in which the machine learning models we
are targeting operate, it is important to focus on the threat model behind this
attack.  Many works in the literature concerning backdoor attacks adopt the
threat model described in BadNets~\cite{gu_badnets:_2017}, which defined:
\begin{enumerate*}[label=(\roman*)]

    \item an \say{Outsourced Training Attack}, where the adversary has full
        control over the training procedure, and the end user is only allowed
        to check the training using a held-out validation dataset;

    \item a \say{Transfer Learning Attack}, in which the user downloads a
        pre-trained model and fine-tunes it.

\end{enumerate*} We argue that, in the context we are examining, this threat
model is difficult to apply directly.   Security companies are generally
extremely protective regarding their intellectual properties, and prefer to
either perform the training in-house, or, at most, outsource the hardware while
maintaining full control over the software stack used during training.  This
attitude protects to a large degree against \say{Outsourced Training Attacks},
and renders \say{Transfer Learning Attacks} almost impossible, at least in the
form in which these attacks were originally devised. Similarly, we don't
believe the threat model used in \cite{liu_trojaning_2018}, where the attacker
is granted the ability to partially retrain the model, applies in this
scenario.

On the other hand, these companies often rely on third parties to acquire
labeled training data, and the screening process for the incoming flow is made
remarkably hard by both the sheer quantities involved, and the intrinsic
difficulty of the task, requiring specialized personnel and software. We,
therefore, target this quite natural weak point in the training pipeline, by
modeling an adversary who leverages crowd-sourced threat streams to disseminate
their poisoned samples.  This adversary takes advantage of the aforementioned
intrinsic difficulties in the evaluation of binaries, combined with the huge
variance that often characterize sets of benign binaries, in order to hide
their backdoored points. We will follow the path outlined by
\cite{gu_badnets:_2017,liu_trojaning_2018} to characterize both the goals, and
capabilities, of such an attacker.


\paragraph{Adversary's Goal}

Similarly to most backdoor poisoning settings, the attacker goal is to alter
the training procedure, such that the resulting classifier, $F_{bdr}$, differs
from a regularly trained classifier $F_{clean}$, where $F_{clean}, F_{bdr}: X
\in \mathbb{R}^{n} \rightarrow \{0,1\}$.  An ideal $F_{bdr}$ would have the
same exact response to a clean set of inputs $X_{clean}$ as $F_{clean}$,
whereas it would generate a different, adversarially chosen, prediction when
applied to a suitably modified set of inputs, $X_{bdr}$. Here $X$, $X_{clean}$,
and $X_{bdr}$ are all testing data points.

\begin{align}
& F_{bdr}(X_{clean}) = F_{clean}(X_{clean}) \nonumber \\
& F_{clean}(X_{bdr}) = y_{clean} \nonumber \\
& F_{bdr}(X_{bdr}) = y_{target} \neq y_{clean}
\end{align}

While in the case of images, and text, there is a concrete difference between
\emph{targeted}, where the adversary's objective is to induce the model to
classify a backdoored input as belonging to a specific target class, and
\emph{non-targeted}, where the aim is just to make the classifier fail to
produce a correct prediction, this difference looses in meaningfulness in the
context of malware detection.  Here, the opponent is almost exclusively
interested in making a malicious binary appear benign, and therefore the target
result is always $y_{target} = 0$. We will assume the class of \emph{benign}
software to be class 0, and that of \emph{malicious} software to be class 1, as
is commonly done in literature and in practical applications. A multi-class
setting, where the attacker's goal is to disguise a malware binary of one
family as belonging to another family could be constructed, but we feel that
such a scenario would be of lesser impact in real-world situations, and,
therefore, we will not consider it here.


\paragraph{Adversary's Capabilities}

Usually, in the context of adversarial machine learning, attacks are
distinguished based on the adversary's knowledge.  In white-box attacks, the
adversary has knowledge of the training data, the model architecture, its
hyper-parameters, and its outputs or logits. In black-box attacks, on the
contrary, only restricted subset of the model characteristics, sometimes
including only the outputs, is known.  

We will start by exploring the \baseatk\ scenario, where the adversary is free
to tamper with the training data without any major constraint. Contrary with
the case of computer vision, where the $\ell_p$-norm is commonly used to
characterize the amplitude of the adversarial modification, here the notion of
distance between different feature vectors does not capture the semantic
differences between the actual programs contained in the binaries. To avoid
assigning completely arbitrary (often impossible) values to the attacked
vectors, we therefore limit our attacker's modification to the set of values
actually found in the population of benign samples in the training set. This
scenario allows us to study the attack and expose its main characteristics
under worst-case conditions.

Then, we constrain the attacker by removing access to the actual target model,
\transferatk, which necessarily forces the attacker to conduct all the
necessary computation on a surrogate model. We note that, despite this scenario
is generally considered black-box in the domain of image classification, in the
context of feature-based models this is not a completely black-box attack since
the adversary still needs to have knowledge of the semantics of the feature set
employed by the target model.  Finally, we will focus on a more realistic
scenario, \feasibleatk, where the adversary is strictly constrained in both the
features of the data points that they are allowed to alter, and the range of
values to employ.  This scenario models the capabilities of a dedicated
attacker with access to the data, who wishes to preserve the programs original
behavior over the alterations in the binaries. A detailed explanation of our
feasibility study is provided in \Cref{feasible}. A quick summary of the attack
scenarios we consider in this work is provided in \Cref{tab:attacker}.


\subsection{Goals and Challenges}

%\alina{These can be integrated into Section 4. I recommend that we highlight the main technical challenges and the main insights more in Section 4.}

%\alina{Figure 1 should include multiple parties contributing data to training, the adversary only controls a subset of samples. Should think about this more.}
To summarize, our design goals are the following: 
\begin{enumerate*}
	\item Insert a small number of watermarked poisoning points at training with the goal of changing the classification of watermarked malware binaries in testing;
	\item Create \emph{clean-label} attacks, in which the watermark is applied to goodware files at training;
	\item Design model agnostic attacks that are applicable to different ML models;
	\item Generate watermarked poisoned points that are not detectable during the training phase by using a clean malware classifier model;
	\item Design attacks feasible to mount in practice by modifying existing Windows PE files. 
\end{enumerate*}

Designing attacks with these properties raises a number of technical challenges. First, selecting the exact features and feature values for the watermark creation becomes difficult given the goal of maintaining attack stealthiness. The model-agnostic requirement excludes methods that are specific to certain ML algorithms, such as using feature importance computed by ensemble models. Practical feasibility is difficult to achieve for attacks modifying PE files, while preserving their functionality. Lastly, the watermark should be applicable to both goodware files in training given the clean-label requirement, and to malware files in testing to enable the successful execution of the attack.

%- Defenses are difficult to design because data has many natural clusters of high density (e.g., legitimate files sharing a subset of features).

% TODO: find a way to structure this section

